How Players Play Games: Observing the Influences of Game Mechanics

The popularity of computer games is remarkably high and is still growing every year. Despite this popularity and the economical importance of gaming, research in game design, or to be more precise, of game mechanics that can be used to improve the enjoyment of a game, is still scarce. In this paper, we analyze Fortnite, one of the currently most successful games, and observe how players play the game. We investigate what makes playing the game enjoyable by analyzing video streams of experienced players from game streaming platforms and by conducting a user study with players who are new to the game. We formulate four hypotheses about how game mechanics influence the way players interact with the game and how it influences player enjoyment. We present differences in player behavior between experienced players and beginners and discuss how game mechanics could be used to improve the enjoyment for beginners. In addition, we describe our approach to analyze games without access to game-internal data by using a toolchain which automatically extracts game information from video streams.

==> content/abstract.tex <==
The popularity of computer games is remarkably high and is still growing every year. Despite this popularity and the economical importance of gaming, research in game design, or to be more precise, of game mechanics %-- game elements and rules defining how a game works -- 
that can be used to improve the enjoyment of a game, is still scarce. In this paper, we analyze \emph{Fortnite}, one of the currently most successful games, and observe how players play the game. We investigate what  makes playing the game enjoyable by analyzing video streams of experienced players from game streaming platforms and by conducting a user study with players who are new to the game. We formulate four hypotheses about how game mechanics influence the way players interact with the game and how it influences player enjoyment. We present differences in player behavior between experienced players and beginners and discuss how game mechanics could be used to improve the enjoyment for beginners. In addition, we describe our approach to analyze games without access to game-internal data by using a toolchain which automatically extracts game information from video streams. 

%, which are used to analyze the influence of game mechanics on player behavior and  To be able to analyze the game, an approach to automatically analyze player behavior from video streams is used and explained in detail. This approach enables researchers be
